Pulsar timing array signals induced by black hole binaries in relativistic eccentric orbits

Individual supermassive black hole binaries in non-circular orbits are possible nanohertz gravitational wave sources for the rapidly maturing Pulsar Timing Array experiments. We develop an accurate and efficient approach to compute Pulsar Timing Array signals due to gravitational waves from inspiraling supermassive black hole binaries in relativistic eccentric orbits. Our approach employs a Keplerian-type parametric solution to model third post-Newtonian accurate precessing eccentric orbits while a novel semi-analytic prescription is provided to model the effects of quadrupolar order gravitational wave emission. These inputs lead to a semi-analytic prescription to model such signals, induced by non-spinning black hole binaries inspiralling along arbitrary eccentricity orbits. Additionally, we provide a fully analytic prescription to model Pulsar Timing Array signals from black hole binaries inspiraling along moderately eccentric orbits, influenced by Boetzelet al.[Phys. Rev. D 96,044011(2017)]. These approaches are being incorporated into Enterprise and TEMPO2 for searching the presence of such binaries in Pulsar Timing Array datasets.

==> hpsp.tex <==
\begin{align}
h_{+} & =H_{0}\Bigg[\left(es_{i}^{2}-\frac{1}{8}e^{3}s_{i}^{2}\right)\cos(l)+\left(e^{2}s_{i}^{2}-\frac{1}{3}e^{4}s_{i}^{2}\right)\cos(2l)\nonumber\\
 & \quad+\left(-\frac{1}{8}23e^{4}c_{i}^{2}+5e^{2}c_{i}^{2}-2c_{i}^{2}-\frac{23e^{4}}{8}+5e^{2}-2\right)\cos(2\lambda)\\
 & \quad+\left(\frac{1}{8}e^{4}c_{i}^{2}+\frac{e^{4}}{8}\right)\cos(4l-2\lambda)+\left(-\frac{1}{4}81e^{4}c_{i}^{2}-\frac{81e^{4}}{4}\right)\cos(2\lambda+4l)\\
 & \quad+\left(\frac{171}{16}e^{3}c_{i}^{2}-\frac{9ec_{i}^{2}}{2}+\frac{171e^{3}}{16}-\frac{9e}{2}\right)\cos(2\lambda+l)+\left(\frac{7}{48}e^{3}c_{i}^{2}+\frac{7e^{3}}{48}\right)\cos(3l-2\lambda)\\
 & \quad+\left(-\frac{1}{16}13e^{3}c_{i}^{2}+\frac{3ec_{i}^{2}}{2}-\frac{13e^{3}}{16}+\frac{3e}{2}\right)\cos(l-2\lambda)\\
 & \quad+\left(-\frac{1}{48}625e^{3}c_{i}^{2}-\frac{625e^{3}}{48}\right)\cos(2\lambda+3l)\\
 & \quad+\left(20e^{4}c_{i}^{2}-8e^{2}c_{i}^{2}+20e^{4}-8e^{2}\right)\cos(2\lambda+2l)\\
 & \quad+\frac{9}{8}e^{3}s_{i}^{2}\cos(3l)+\frac{4}{3}e^{4}s_{i}^{2}\cos(4l)\Bigg]\\
s_{+} & =\frac{H_{0}}{n}\Bigg[\;\left(es_{i}^{2}-\frac{1}{8}e^{3}s_{i}^{2}\right)\sin(l)+\left(\frac{1}{2}e^{2}s_{i}^{2}-\frac{1}{6}e^{4}s_{i}^{2}\right)\sin(2l)\\
 & \quad+\left(-\frac{1}{16}23e^{4}c_{i}^{2}+\frac{5}{2}e^{2}c_{i}^{2}-c_{i}^{2}-\frac{23e^{4}}{16}+\frac{5e^{2}}{2}-1\right)\sin(2\lambda)\\
 & \quad+\left(\frac{13}{16}e^{3}c_{i}^{2}-\frac{3ec_{i}^{2}}{2}+\frac{13e^{3}}{16}-\frac{3e}{2}\right)\sin(l-2\lambda)\\
 & \quad+\left(\frac{57}{16}e^{3}c_{i}^{2}-\frac{3ec_{i}^{2}}{2}+\frac{57e^{3}}{16}-\frac{3e}{2}\right)\sin(2\lambda+l)\\
 & \quad+\left(\frac{1}{16}e^{4}c_{i}^{2}+\frac{e^{4}}{16}\right)\sin(4l-2\lambda)+\left(-\frac{1}{8}27e^{4}c_{i}^{2}-\frac{27e^{4}}{8}\right)\sin(2\lambda+4l)\\
 & \quad+\left(\frac{7}{48}e^{3}c_{i}^{2}+\frac{7e^{3}}{48}\right)\sin(3l-2\lambda)+\left(-\frac{1}{48}125e^{3}c_{i}^{2}-\frac{125e^{3}}{48}\right)\sin(2\lambda+3l)\\
 & \quad+\left(5e^{4}c_{i}^{2}-2e^{2}c_{i}^{2}+5e^{4}-2e^{2}\right)\sin(2\lambda+2l)\\
 & \quad+\frac{1}{3}e^{4}s_{i}^{2}\sin(4l)+\frac{3}{8}e^{3}s_{i}^{2}\sin(3l)\;\Bigg]
\end{align}
